Antihydrogen Formation, Trapping and Dynamics

Antihydrogen, the simplest pure-antimatter atomic system, holds the promise of direct tests of matter-antimatter equivalence and CPT invariance, two of the outstanding unanswered questions in modern physics. Antihydrogen is now routinely produced in charged-particle traps through the combination of plasmas of antiprotons and positrons, but the atoms escape and are destroyed in a minuscule fraction of a second. The focus of this work is the production of a sample of cold antihydrogen atoms in a magnetic atom trap. This poses an extreme challenge, because the state-of-the-art atom traps are only approximately 0.5 K deep for ground-state antihydrogen atoms, much shallower than the energies of particles stored in the plasmas. This thesis will outline the main parts of the ALPHA experiment, with an overview of the important physical processes at work. Antihydrogen production techniques will be described, and an analysis of the spatial annihilation distribution to give indications of the temperature and binding energy distribution of the atoms will be presented. Finally, we describe the techniques needed to demonstrate confinement of antihydrogen atoms, apply them to a data taking run and present the results, making a definitive identification of trapped antihydrogen atoms.

==> chap_cooling/EVCCooling.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,4320.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1308,1259){\makebox(0,0)[r]{\strut{} 10}}%
      \put(1308,2573){\makebox(0,0)[r]{\strut{} 100}}%
      \put(1308,3887){\makebox(0,0)[r]{\strut{} 1000}}%
      \put(2146,644){\makebox(0,0){\strut{} 10}}%
      \put(4493,644){\makebox(0,0){\strut{} 100}}%
      \put(6839,644){\makebox(0,0){\strut{} 1000}}%
      \put(406,2375){\rotatebox{-270}{\makebox(0,0){\strut{}Temperature [K]}}}%
      \put(4139,314){\makebox(0,0){\strut{}Well depth [mV]}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{chap_cooling/EVCCooling}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> chap_hbar/ARSweepCompare.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1668,576){\makebox(0,0)[r]{\strut{} 0}}%
      \put(1668,1248){\makebox(0,0)[r]{\strut{} 0.2}}%
      \put(1668,1919){\makebox(0,0)[r]{\strut{} 0.4}}%
      \put(1668,2591){\makebox(0,0)[r]{\strut{} 0.6}}%
      \put(1800,356){\makebox(0,0){\strut{} 0}}%
      \put(2808,356){\makebox(0,0){\strut{} 0.5}}%
      \put(3816,356){\makebox(0,0){\strut{} 1}}%
      \put(4823,356){\makebox(0,0){\strut{} 1.5}}%
      \put(5831,356){\makebox(0,0){\strut{} 2}}%
      \put(6839,356){\makebox(0,0){\strut{} 2.5}}%
      \put(898,1583){\rotatebox{-270}{\makebox(0,0){\strut{}Accumulated Charge [Arb]}}}%
      \put(4319,26){\makebox(0,0){\strut{}Time [ms]}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5852,2418){\makebox(0,0)[r]{\strut{}100\%}}%
      \csname LTb\endcsname%
      \put(5852,2198){\makebox(0,0)[r]{\strut{}50\%}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{chap_hbar/ARSweepCompare}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> chap_hbar/ARSweepCompareTriggers.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1668,576){\makebox(0,0)[r]{\strut{} 0}}%
      \put(1668,1248){\makebox(0,0)[r]{\strut{} 1000}}%
      \put(1668,1919){\makebox(0,0)[r]{\strut{} 2000}}%
      \put(1668,2591){\makebox(0,0)[r]{\strut{} 3000}}%
      \put(2258,356){\makebox(0,0){\strut{} 0}}%
      \put(3174,356){\makebox(0,0){\strut{} 0.2}}%
      \put(4090,356){\makebox(0,0){\strut{} 0.4}}%
      \put(5007,356){\makebox(0,0){\strut{} 0.6}}%
      \put(5923,356){\makebox(0,0){\strut{} 0.8}}%
      \put(6839,356){\makebox(0,0){\strut{} 1}}%
      \put(766,1583){\rotatebox{-270}{\makebox(0,0){\strut{}Integrated annihilation counts}}}%
      \put(4319,26){\makebox(0,0){\strut{}Time [s]}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2787,2418){\makebox(0,0)[l]{\strut{}Nominal}}%
      \csname LTb\endcsname%
      \put(2787,2198){\makebox(0,0)[l]{\strut{}50\%}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{chap_hbar/ARSweepCompareTriggers}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> chap_hbar/ArMixingPotential.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,3600.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1308,720){\makebox(0,0)[r]{\strut{}-6}}%
      \put(1308,1140){\makebox(0,0)[r]{\strut{}-5}}%
      \put(1308,1560){\makebox(0,0)[r]{\strut{}-4}}%
      \put(1308,1979){\makebox(0,0)[r]{\strut{}-3}}%
      \put(1308,2399){\makebox(0,0)[r]{\strut{}-2}}%
      \put(1308,2819){\makebox(0,0)[r]{\strut{}-1}}%
      \put(1308,3239){\makebox(0,0)[r]{\strut{} 0}}%
      \put(1440,500){\makebox(0,0){\strut{} 0.3}}%
      \put(2491,500){\makebox(0,0){\strut{} 0.35}}%
      \put(3542,500){\makebox(0,0){\strut{} 0.4}}%
      \put(4593,500){\makebox(0,0){\strut{} 0.45}}%
      \put(5644,500){\makebox(0,0){\strut{} 0.5}}%
      \put(6695,500){\makebox(0,0){\strut{} 0.55}}%
      \put(802,1979){\rotatebox{-270}{\makebox(0,0){\strut{}Potnetial [V]}}}%
      \put(4067,170){\makebox(0,0){\strut{}z [m]}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5708,3066){\makebox(0,0)[r]{\strut{}with positron plasma}}%
      \csname LTb\endcsname%
      \put(5708,2846){\makebox(0,0)[r]{\strut{}ignoring positron plasma}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{chap_hbar/ArMixingPotential}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> chap_hbar/hbarvertices.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7920.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3326,4492){\makebox(0,0)[l]{\strut{}(b)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4124,1470){\makebox(0,0){\strut{}-10}}%
      \put(5032,1470){\makebox(0,0){\strut{}-5}}%
      \put(5939,1470){\makebox(0,0){\strut{} 0}}%
      \put(6846,1470){\makebox(0,0){\strut{} 5}}%
      \put(7754,1470){\makebox(0,0){\strut{} 10}}%
      \put(5939,1140){\makebox(0,0){\strut{}z [cm]}}%
      \put(3952,1756){\makebox(0,0)[r]{\strut{}$\pi$}}%
      \put(3952,2373){\makebox(0,0)[r]{\strut{}$-\pi/2$}}%
      \put(3952,2989){\makebox(0,0)[r]{\strut{}0}}%
      \put(3952,3605){\makebox(0,0)[r]{\strut{}$\pi/2$}}%
      \put(3952,4222){\makebox(0,0)[r]{\strut{}$-\pi$}}%
      \put(3490,2989){\rotatebox{-270}{\makebox(0,0){\strut{}$\phi$}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \put(158,4492){\makebox(0,0)[l]{\strut{}(a)}}%
      \put(3326,4492){\makebox(0,0)[l]{\strut{}(b)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(918,1477){\makebox(0,0){\strut{}-4}}%
      \put(1409,1477){\makebox(0,0){\strut{}-2}}%
      \put(1900,1477){\makebox(0,0){\strut{} 0}}%
      \put(2391,1477){\makebox(0,0){\strut{} 2}}%
      \put(2882,1477){\makebox(0,0){\strut{} 4}}%
      \put(1900,1147){\makebox(0,0){\strut{}x [cm]}}%
      \put(501,2008){\makebox(0,0)[r]{\strut{}-4}}%
      \put(501,2499){\makebox(0,0)[r]{\strut{}-2}}%
      \put(501,2990){\makebox(0,0)[r]{\strut{}0}}%
      \put(501,3481){\makebox(0,0)[r]{\strut{}2}}%
      \put(501,3972){\makebox(0,0)[r]{\strut{}4}}%
      \put(171,2990){\rotatebox{-270}{\makebox(0,0){\strut{}y [cm]}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{chap_hbar/hbarvertices}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> chap_hbar/hotSpots.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7920.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3326,4492){\makebox(0,0)[l]{\strut{}(b)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4124,1470){\makebox(0,0){\strut{}-10}}%
      \put(5032,1470){\makebox(0,0){\strut{}-5}}%
      \put(5939,1470){\makebox(0,0){\strut{} 0}}%
      \put(6846,1470){\makebox(0,0){\strut{} 5}}%
      \put(7754,1470){\makebox(0,0){\strut{} 10}}%
      \put(5939,1140){\makebox(0,0){\strut{}z [cm]}}%
      \put(3952,1756){\makebox(0,0)[r]{\strut{}$\pi$}}%
      \put(3952,2373){\makebox(0,0)[r]{\strut{}$-\pi/2$}}%
      \put(3952,2989){\makebox(0,0)[r]{\strut{}0}}%
      \put(3952,3605){\makebox(0,0)[r]{\strut{}$\pi/2$}}%
      \put(3952,4222){\makebox(0,0)[r]{\strut{}$-\pi$}}%
      \put(3490,2989){\rotatebox{-270}{\makebox(0,0){\strut{}$\phi$}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \put(158,4492){\makebox(0,0)[l]{\strut{}(a)}}%
      \put(3326,4492){\makebox(0,0)[l]{\strut{}(b)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(918,1477){\makebox(0,0){\strut{}-4}}%
      \put(1409,1477){\makebox(0,0){\strut{}-2}}%
      \put(1900,1477){\makebox(0,0){\strut{} 0}}%
      \put(2391,1477){\makebox(0,0){\strut{} 2}}%
      \put(2882,1477){\makebox(0,0){\strut{} 4}}%
      \put(1900,1147){\makebox(0,0){\strut{}x [cm]}}%
      \put(501,2008){\makebox(0,0)[r]{\strut{}-4}}%
      \put(501,2499){\makebox(0,0)[r]{\strut{}-2}}%
      \put(501,2990){\makebox(0,0)[r]{\strut{}0}}%
      \put(501,3481){\makebox(0,0)[r]{\strut{}2}}%
      \put(501,3972){\makebox(0,0)[r]{\strut{}4}}%
      \put(171,2990){\rotatebox{-270}{\makebox(0,0){\strut{}y [cm]}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{chap_hbar/hotSpots}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> chap_isotrop/bestOffset.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,2448.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1308,489){\makebox(0,0)[r]{\strut{} 0}}%
      \put(1308,717){\makebox(0,0)[r]{\strut{} 2000}}%
      \put(1308,946){\makebox(0,0)[r]{\strut{} 4000}}%
      \put(1308,1174){\makebox(0,0)[r]{\strut{} 6000}}%
      \put(1308,1403){\makebox(0,0)[r]{\strut{} 8000}}%
      \put(1308,1631){\makebox(0,0)[r]{\strut{} 10000}}%
      \put(1308,1859){\makebox(0,0)[r]{\strut{} 12000}}%
      \put(1308,2088){\makebox(0,0)[r]{\strut{} 14000}}%
      \put(1440,269){\makebox(0,0){\strut{} 100}}%
      \put(3240,269){\makebox(0,0){\strut{} 1000}}%
      \put(5039,269){\makebox(0,0){\strut{} 10000}}%
      \put(6839,269){\makebox(0,0){\strut{} 100000}}%
      \put(274,1345){\rotatebox{-270}{\makebox(0,0){\strut{}$v_0 [\mathrm{m\,s^{-1}}]$}}}%
      \put(4139,-61){\makebox(0,0){\strut{}$T$ [K]}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{chap_isotrop/bestOffset}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> chap_isotrop/bestOffsetChi.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,2448.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1308,489){\makebox(0,0)[r]{\strut{} 0}}%
      \put(1308,679){\makebox(0,0)[r]{\strut{} 20}}%
      \put(1308,870){\makebox(0,0)[r]{\strut{} 40}}%
      \put(1308,1060){\makebox(0,0)[r]{\strut{} 60}}%
      \put(1308,1250){\makebox(0,0)[r]{\strut{} 80}}%
      \put(1308,1441){\makebox(0,0)[r]{\strut{} 100}}%
      \put(1308,1631){\makebox(0,0)[r]{\strut{} 120}}%
      \put(1308,1821){\makebox(0,0)[r]{\strut{} 140}}%
      \put(1308,2012){\makebox(0,0)[r]{\strut{} 160}}%
      \put(1308,2202){\makebox(0,0)[r]{\strut{} 180}}%
      \put(1440,269){\makebox(0,0){\strut{} 100}}%
      \put(3240,269){\makebox(0,0){\strut{} 1000}}%
      \put(5039,269){\makebox(0,0){\strut{} 10000}}%
      \put(6839,269){\makebox(0,0){\strut{} 100000}}%
      \put(538,1345){\rotatebox{-270}{\makebox(0,0){\strut{}$\chi^2$}}}%
      \put(4139,-61){\makebox(0,0){\strut{}$T$ [K]}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{chap_isotrop/bestOffsetChi}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> chap_isotrop/bestOffsetNorm.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,2448.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1308,489){\makebox(0,0)[r]{\strut{} 0}}%
      \put(1308,775){\makebox(0,0)[r]{\strut{} 0.5}}%
      \put(1308,1060){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1308,1346){\makebox(0,0)[r]{\strut{} 1.5}}%
      \put(1308,1631){\makebox(0,0)[r]{\strut{} 2}}%
      \put(1308,1917){\makebox(0,0)[r]{\strut{} 2.5}}%
      \put(1308,2202){\makebox(0,0)[r]{\strut{} 3}}%
      \put(1440,269){\makebox(0,0){\strut{} 100}}%
      \put(3240,269){\makebox(0,0){\strut{} 1000}}%
      \put(5039,269){\makebox(0,0){\strut{} 10000}}%
      \put(6839,269){\makebox(0,0){\strut{} 100000}}%
      \put(538,1345){\rotatebox{-270}{\makebox(0,0){\strut{}$v_0/\frac{k_\mathrm{B}T}{m}$}}}%
      \put(4139,-61){\makebox(0,0){\strut{}$T$ [K]}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{chap_isotrop/bestOffsetNorm}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> chap_isotrop/dump.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(418,704){\makebox(0,0)[r]{\strut{}}}%
      \put(418,1213){\makebox(0,0)[r]{\strut{}}}%
      \put(418,1722){\makebox(0,0)[r]{\strut{}}}%
      \put(418,2231){\makebox(0,0)[r]{\strut{}}}%
      \put(418,2740){\makebox(0,0)[r]{\strut{}}}%
      \put(418,3248){\makebox(0,0)[r]{\strut{}}}%
      \put(418,3757){\makebox(0,0)[r]{\strut{}}}%
      \put(418,4266){\makebox(0,0)[r]{\strut{}}}%
      \put(418,4775){\makebox(0,0)[r]{\strut{}}}%
      \put(918,484){\makebox(0,0){\strut{}-0.15}}%
      \put(1837,484){\makebox(0,0){\strut{}-0.1}}%
      \put(2757,484){\makebox(0,0){\strut{}-0.05}}%
      \put(3676,484){\makebox(0,0){\strut{} 0}}%
      \put(4596,484){\makebox(0,0){\strut{} 0.05}}%
      \put(5516,484){\makebox(0,0){\strut{} 0.1}}%
      \put(6435,484){\makebox(0,0){\strut{} 0.15}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Number of vertices [arb]}}}%
      \put(3676,154){\makebox(0,0){\strut{}Z Position [m]}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5816,4602){\makebox(0,0)[r]{\strut{}2009-1}}%
      \csname LTb\endcsname%
      \put(5816,4382){\makebox(0,0)[r]{\strut{}2009-2}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(418,704){\makebox(0,0)[r]{\strut{}}}%
      \put(418,1167){\makebox(0,0)[r]{\strut{}}}%
      \put(418,1629){\makebox(0,0)[r]{\strut{}}}%
      \put(418,2092){\makebox(0,0)[r]{\strut{}}}%
      \put(418,2554){\makebox(0,0)[r]{\strut{}}}%
      \put(418,3017){\makebox(0,0)[r]{\strut{}}}%
      \put(418,3480){\makebox(0,0)[r]{\strut{}}}%
      \put(418,3942){\makebox(0,0)[r]{\strut{}}}%
      \put(418,4405){\makebox(0,0)[r]{\strut{}}}%
      \put(918,484){\makebox(0,0){\strut{}-0.15}}%
      \put(1837,484){\makebox(0,0){\strut{}-0.1}}%
      \put(2757,484){\makebox(0,0){\strut{}-0.05}}%
      \put(3676,484){\makebox(0,0){\strut{} 0}}%
      \put(4596,484){\makebox(0,0){\strut{} 0.05}}%
      \put(5516,484){\makebox(0,0){\strut{} 0.1}}%
      \put(6435,484){\makebox(0,0){\strut{} 0.15}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Number of vertices [arb]}}}%
      \put(3676,154){\makebox(0,0){\strut{}Z Position [m]}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5816,4602){\makebox(0,0)[r]{\strut{}2009-1}}%
      \csname LTb\endcsname%
      \put(5816,4382){\makebox(0,0)[r]{\strut{}2009-2}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{chap_isotrop/dump}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> chap_isotrop/epithermaldist.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,3600.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(4068,500){\makebox(0,0){\strut{} 0}}%
      \put(4067,170){\makebox(0,0){\strut{}v}}%
      \colorrgb{0.00,0.00,0.00}%
      \put(3752,2740){\makebox(0,0)[r]{\strut{}$\sqrt{\frac{k_\mathrm{B}T}{m}}$}}%
      \colorrgb{1.00,0.00,0.00}%
      \put(4330,1351){\makebox(0,0){\strut{}$v_0$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5708,3066){\makebox(0,0)[r]{\strut{}thermal}}%
      \csname LTb\endcsname%
      \put(5708,2846){\makebox(0,0)[r]{\strut{}epithermal}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{chap_isotrop/epithermaldist}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> chap_isotrop/null.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,4320.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(947,864){\makebox(0,0)[r]{\strut{}}}%
      \put(947,1469){\makebox(0,0)[r]{\strut{}}}%
      \put(947,2073){\makebox(0,0)[r]{\strut{}}}%
      \put(947,2678){\makebox(0,0)[r]{\strut{}}}%
      \put(947,3282){\makebox(0,0)[r]{\strut{}}}%
      \put(947,3887){\makebox(0,0)[r]{\strut{}}}%
      \put(1727,644){\makebox(0,0){\strut{}-0.1}}%
      \put(2807,644){\makebox(0,0){\strut{}-0.05}}%
      \put(3887,644){\makebox(0,0){\strut{} 0}}%
      \put(4967,644){\makebox(0,0){\strut{} 0.05}}%
      \put(6047,644){\makebox(0,0){\strut{} 0.1}}%
      \put(705,2375){\rotatebox{-270}{\makebox(0,0){\strut{}Number of vertices [arb]}}}%
      \put(3887,314){\makebox(0,0){\strut{}z [m]}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5708,3714){\makebox(0,0)[r]{\strut{}S. Jonsell}}%
      \csname LTb\endcsname%
      \put(5708,3494){\makebox(0,0)[r]{\strut{}$a=1.5$}}%
      \csname LTb\endcsname%
      \put(5708,3274){\makebox(0,0)[r]{\strut{}$a=2.0$}}%
      \csname LTb\endcsname%
      \put(5708,3054){\makebox(0,0)[r]{\strut{}$a=3.0$}}%
      \csname LTb\endcsname%
      \put(5708,2834){\makebox(0,0)[r]{\strut{}2009-2 data}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(947,864){\makebox(0,0)[r]{\strut{}}}%
      \put(947,1440){\makebox(0,0)[r]{\strut{}}}%
      \put(947,2016){\makebox(0,0)[r]{\strut{}}}%
      \put(947,2591){\makebox(0,0)[r]{\strut{}}}%
      \put(947,3167){\makebox(0,0)[r]{\strut{}}}%
      \put(947,3743){\makebox(0,0)[r]{\strut{}}}%
      \put(1727,644){\makebox(0,0){\strut{}-0.1}}%
      \put(2807,644){\makebox(0,0){\strut{}-0.05}}%
      \put(3887,644){\makebox(0,0){\strut{} 0}}%
      \put(4967,644){\makebox(0,0){\strut{} 0.05}}%
      \put(6047,644){\makebox(0,0){\strut{} 0.1}}%
      \put(705,2375){\rotatebox{-270}{\makebox(0,0){\strut{}Number of vertices [arb]}}}%
      \put(3887,314){\makebox(0,0){\strut{}z [m]}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5708,3714){\makebox(0,0)[r]{\strut{}S. Jonsell}}%
      \csname LTb\endcsname%
      \put(5708,3494){\makebox(0,0)[r]{\strut{}$a=1.5$}}%
      \csname LTb\endcsname%
      \put(5708,3274){\makebox(0,0)[r]{\strut{}$a=2.0$}}%
      \csname LTb\endcsname%
      \put(5708,3054){\makebox(0,0)[r]{\strut{}$a=3.0$}}%
      \csname LTb\endcsname%
      \put(5708,2834){\makebox(0,0)[r]{\strut{}2009-2 data}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{chap_isotrop/null}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> chap_isotrop/offests.tex <==

\subsection{The influence of the formation position}
The position at which recombination occurs can also have an effect on the annihilation distribution.







The size of the positron plasma is sufficiently small compared to the size of the trap that the change in the initial position ($\mathbf{r}_0$) in equation \ref{eq:z_annihilation} of the atom has little influence on where it annihilates -- the positron plasma is well-approximated by a point source.
Instead, the main effect of a change in the formation position is the change in contribution of the $\mathbf{E}\times\mathbf{B}$ velocity, which varies as a function of radial position, as shown in figure \ref{fig:isotrop_vr}.
At 120~K, the thermal velocity of $\sim 800\mathrm{m\,s^{-1}}$ is comparable to the maximum rotational speed of $\sim 600~\mathrm{m\,s^{-1}}$, so the $\mathbf{E}\times\mathbf{B}$ velocity plays a significant, though not dominant role.

On the axis of the trap the rotational speed is zero, and this distribution is practically the same as the high-temperature, isotropic distributions discussed in the previous section.
This is the distribution that best matches the measurements, but using this distribution would disagree with the MCP/Phosphor measurements.



\clearpage
\newpage




==> chap_isotrop/s2_kappascan.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,4320.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(814,704){\makebox(0,0)[r]{\strut{} 1}}%
      \put(814,1263){\makebox(0,0)[r]{\strut{} 2}}%
      \put(814,1821){\makebox(0,0)[r]{\strut{} 3}}%
      \put(814,2380){\makebox(0,0)[r]{\strut{} 4}}%
      \put(814,2938){\makebox(0,0)[r]{\strut{} 5}}%
      \put(814,3497){\makebox(0,0)[r]{\strut{} 6}}%
      \put(814,4055){\makebox(0,0)[r]{\strut{} 7}}%
      \put(1316,484){\makebox(0,0){\strut{} 0.5}}%
      \put(1933,484){\makebox(0,0){\strut{} 1}}%
      \put(2550,484){\makebox(0,0){\strut{} 1.5}}%
      \put(3167,484){\makebox(0,0){\strut{} 2}}%
      \put(3784,484){\makebox(0,0){\strut{} 2.5}}%
      \put(4401,484){\makebox(0,0){\strut{} 3}}%
      \put(5018,484){\makebox(0,0){\strut{} 3.5}}%
      \put(5635,484){\makebox(0,0){\strut{} 4}}%
      \put(6252,484){\makebox(0,0){\strut{} 4.5}}%
      \put(6869,484){\makebox(0,0){\strut{} 5}}%
      \put(308,2379){\rotatebox{-270}{\makebox(0,0){\strut{}$\Chi^2/\mathrm{ndf}$}}}%
      \put(3907,154){\makebox(0,0){\strut{}$\kappa$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(2298,2961){\makebox(0,0)[r]{\strut{} 1.6}}%
      \put(2298,3424){\makebox(0,0)[r]{\strut{} 1.7}}%
      \put(2298,3887){\makebox(0,0)[r]{\strut{} 1.8}}%
      \put(2918,2509){\makebox(0,0){\strut{} 1.2}}%
      \put(3569,2509){\makebox(0,0){\strut{} 1.4}}%
      \put(4221,2509){\makebox(0,0){\strut{} 1.6}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{chap_isotrop/s2_kappascan}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> chap_trap/unnamed.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{unnamed}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           02-Dec-2010 16:58:27
% eps bounding box:     15 cm x 6 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s08}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Potential\end{tabular}}%
\psfrag{s09}[l][l]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}(a)\end{tabular}}%
\psfrag{s10}[l][l]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}(b)\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{0.05}%
\psfrag{x02}[t][t]{0.1}%
\psfrag{x03}[t][t]{0.15}%
\psfrag{x04}[t][t]{0.2}%
\psfrag{x05}[t][t]{0.05}%
\psfrag{x06}[t][t]{0.1}%
\psfrag{x07}[t][t]{0.15}%
\psfrag{x08}[t][t]{0.2}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{10}%
\psfrag{v03}[r][r]{20}%
\psfrag{v04}[r][r]{30}%
\psfrag{v05}[r][r]{40}%
\psfrag{v06}[r][r]{50}%
\psfrag{v07}[r][r]{60}%
%
% Figure:
\resizebox{12cm}{!}{\includegraphics{unnamed.eps}}%
\end{psfrags}%
%
% End unnamed.tex


==> chap_trapping/miirorTrapevents.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(947,576){\makebox(0,0)[r]{\strut{} 0}}%
      \put(947,1248){\makebox(0,0)[r]{\strut{} 10}}%
      \put(947,1919){\makebox(0,0)[r]{\strut{} 20}}%
      \put(947,2591){\makebox(0,0)[r]{\strut{} 30}}%
      \put(1655,356){\makebox(0,0){\strut{}-0.2}}%
      \put(2807,356){\makebox(0,0){\strut{}-0.1}}%
      \put(3959,356){\makebox(0,0){\strut{} 0}}%
      \put(5111,356){\makebox(0,0){\strut{} 0.1}}%
      \put(6263,356){\makebox(0,0){\strut{} 0.2}}%
      \put(309,1583){\rotatebox{-270}{\makebox(0,0){\strut{}t [ms]}}}%
      \put(3959,26){\makebox(0,0){\strut{}z [m]}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(947,576){\makebox(0,0)[r]{\strut{} 0}}%
      \put(947,1248){\makebox(0,0)[r]{\strut{} 10}}%
      \put(947,1919){\makebox(0,0)[r]{\strut{} 20}}%
      \put(947,2591){\makebox(0,0)[r]{\strut{} 30}}%
      \put(1655,356){\makebox(0,0){\strut{}-0.2}}%
      \put(2807,356){\makebox(0,0){\strut{}-0.1}}%
      \put(3959,356){\makebox(0,0){\strut{} 0}}%
      \put(5111,356){\makebox(0,0){\strut{} 0.1}}%
      \put(6263,356){\makebox(0,0){\strut{} 0.2}}%
      \put(309,1583){\rotatebox{-270}{\makebox(0,0){\strut{}t [ms]}}}%
      \put(3959,26){\makebox(0,0){\strut{}z [m]}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5852,2418){\makebox(0,0)[r]{\strut{}No bias}}%
      \csname LTb\endcsname%
      \put(5852,2198){\makebox(0,0)[r]{\strut{}Left bias}}%
      \csname LTb\endcsname%
      \put(5852,1978){\makebox(0,0)[r]{\strut{}Right bias}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{chap_trapping/miirorTrapevents}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> chap_vertex/dump.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,4320.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(418,704){\makebox(0,0)[r]{\strut{}}}%
      \put(418,1123){\makebox(0,0)[r]{\strut{}}}%
      \put(418,1542){\makebox(0,0)[r]{\strut{}}}%
      \put(418,1961){\makebox(0,0)[r]{\strut{}}}%
      \put(418,2380){\makebox(0,0)[r]{\strut{}}}%
      \put(418,2798){\makebox(0,0)[r]{\strut{}}}%
      \put(418,3217){\makebox(0,0)[r]{\strut{}}}%
      \put(418,3636){\makebox(0,0)[r]{\strut{}}}%
      \put(418,4055){\makebox(0,0)[r]{\strut{}}}%
      \put(1271,484){\makebox(0,0){\strut{}-0.1}}%
      \put(2474,484){\makebox(0,0){\strut{}-0.05}}%
      \put(3676,484){\makebox(0,0){\strut{} 0}}%
      \put(4879,484){\makebox(0,0){\strut{} 0.05}}%
      \put(6081,484){\makebox(0,0){\strut{} 0.1}}%
      \put(176,2379){\rotatebox{-270}{\makebox(0,0){\strut{}Number of vertices [arb]}}}%
      \put(3676,154){\makebox(0,0){\strut{}z [m]}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5816,3882){\makebox(0,0)[r]{\strut{}Combined}}%
      \csname LTb\endcsname%
      \put(5816,3662){\makebox(0,0)[r]{\strut{}Antiproton}}%
      \csname LTb\endcsname%
      \put(5816,3442){\makebox(0,0)[r]{\strut{}Antihydrogen}}%
      \csname LTb\endcsname%
      \put(5816,3222){\makebox(0,0)[r]{\strut{}2009-2 data}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(418,704){\makebox(0,0)[r]{\strut{}}}%
      \put(418,1103){\makebox(0,0)[r]{\strut{}}}%
      \put(418,1502){\makebox(0,0)[r]{\strut{}}}%
      \put(418,1901){\makebox(0,0)[r]{\strut{}}}%
      \put(418,2300){\makebox(0,0)[r]{\strut{}}}%
      \put(418,2699){\makebox(0,0)[r]{\strut{}}}%
      \put(418,3098){\makebox(0,0)[r]{\strut{}}}%
      \put(418,3496){\makebox(0,0)[r]{\strut{}}}%
      \put(418,3895){\makebox(0,0)[r]{\strut{}}}%
      \put(1271,484){\makebox(0,0){\strut{}-0.1}}%
      \put(2474,484){\makebox(0,0){\strut{}-0.05}}%
      \put(3676,484){\makebox(0,0){\strut{} 0}}%
      \put(4879,484){\makebox(0,0){\strut{} 0.05}}%
      \put(6081,484){\makebox(0,0){\strut{} 0.1}}%
      \put(176,2379){\rotatebox{-270}{\makebox(0,0){\strut{}Number of vertices [arb]}}}%
      \put(3676,154){\makebox(0,0){\strut{}z [m]}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5816,3882){\makebox(0,0)[r]{\strut{}Combined}}%
      \csname LTb\endcsname%
      \put(5816,3662){\makebox(0,0)[r]{\strut{}Antiproton}}%
      \csname LTb\endcsname%
      \put(5816,3442){\makebox(0,0)[r]{\strut{}Antihydrogen}}%
      \csname LTb\endcsname%
      \put(5816,3222){\makebox(0,0)[r]{\strut{}2009-2 data}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{/home/ebutler/alpha/thesis/chap_vertex/dump}}%
    \gplfronttext
  \end{picture}%
\endgroup

